RiskLabs: Predicting Financial Risk Using Large Language Model based on Multimodal and Multi-Sources Data

The integration of Artificial Intelligence (AI) techniques, particularly large language models (LLMs), in finance has garnered increasing academic attention. Despite progress, existing studies predominantly focus on tasks like financial text summarization, question-answering, and stock movement prediction (binary classification), the application of LLMs to financial risk prediction remains underexplored. Addressing this gap, in this paper, we introduce RiskLabs, a novel framework that leverages LLMs to analyze and predict financial risks. RiskLabs uniquely integrates multimodal financial data, including textual and vocal information from Earnings Conference Calls (ECCs), market-related time series data, and contextual news data to improve financial risk prediction. Empirical results demonstrate RiskLabs' effectiveness in forecasting both market volatility and variance. Through comparative experiments, we examine the contributions of different data sources to financial risk assessment and highlight the crucial role of LLMs in this process. We also discuss the challenges associated with using LLMs for financial risk prediction and explore the potential of combining them with multimodal data for this purpose.

==> problem.tex <==
\section{Problem Formulation}\label{problem}
RiskLabs is a multi-task training model that trains and predicts the volatility of different terms and VaR. The individual stock volatility can be expressed as the natural log of the standard deviation of return prices \(r\) in a window of \({\tau}\) days. We calculate the 3, 7, 15, and 30 trading days volatility using the equation:
\begin{equation}
\label{e:vol}
v_{[d-\tau, d]} = \ln\left(\left(\frac{\sum_{i=0}^{\tau}(r_{d-i}-\bar{r})^{2}}{\tau}\right)^{\frac{1}{2}}\right) 
\end{equation}
The notations used across the paper are discussed herein. Let \(s \in S\) denote a stock, \(c \in C\) be an earnings call for stock s. For each stock, there exist multiple earnings calls c that are held periodically. Each call c can be segmented into a set of \(a_{c}^i \in A_{c}\) audio clips, and corresponding \(t_{c}^i \in T_{c}\) text sentences for \(i \in [1,N]\), where \(N\) is the maximum number of audio clips in a call. For each stock, there exists a daily return denoted by \(r_i = \ \frac {p_i - p_{i-1}}{p_{i-1}}\), where \(p_i\) is the adjusted close price at the end of the day and \=r is the average return over a period of \({\tau}\) days. We aim to develop a predictive regression function \(f(c) \rightarrow v_{[d-\tau, d]}\)


Our second task is predicting the 1-day VaR of the target stock based on the multi-source inputs. The definition of VaR is:
\begin{align*}
    x = F^{-1}(p)
\end{align*}
The $F(\cdot)$ is the cumulative loss distribution, $p$ is the percentile we set, and $x$ is the VaR. From the idea of Quantile Regression, we can have: 
\begin{align*}
    L_{\tau}(y, \hat{y}) = \begin{cases} 
  \tau \cdot (y - \hat{y}) & \text{if } y \geq \hat{y} \\
  (1 - \tau) \cdot (\hat{y} - y) & \text{if } y < \hat{y} 
\end{cases}
\end{align*}


For the evaluation, following~\cite{qin2019you}, we assess the accuracy of volatility predictions by comparing the predicted volatility values $y_i$ with the true volatility values $\hat{y_i}$. We use Mean Squared Error (MSE) as the evaluation metric:
\begin{equation}
MSE = \frac{\sum_{i}^{m}(y_i - \hat{y_i})^2}{m}
\end{equation}

where $m$ is the size of the test set, this metric quantifies the average squared difference between the predicted and actual volatility values, providing a measure of prediction accuracy. Additionally, for constructing volatility labels, we collected stock price information via the Yahoo Finance API\footnote{https://finance.yahoo.com/} and used equation~\ref{e:vol} to calculate the labels (true volatility values $\hat{y_i}$) for days 3, 7, 15, and 30.

